DDF-HO: Hand-Held Object Reconstruction via Conditional Directed Distance Field

Reconstructing hand-held objects from a single RGB image is an important and challenging problem. Existing works utilizing Signed Distance Fields (SDF) reveal limitations in comprehensively capturing the complex hand-object interactions, since SDF is only reliable within the proximity of the target, and hence, infeasible to simultaneously encode local hand and object cues. To address this issue, we propose DDF-HO, a novel approach leveraging Directed Distance Field (DDF) as the shape representation. Unlike SDF, DDF maps a ray in 3D space, consisting of an origin and a direction, to corresponding DDF values, including a binary visibility signal determining whether the ray intersects the objects and a distance value measuring the distance from origin to target in the given direction. We randomly sample multiple rays and collect local to global geometric features for them by introducing a novel 2D ray-based feature aggregation scheme and a 3D intersection-aware hand pose embedding, combining 2D-3D features to model hand-object interactions. Extensive experiments on synthetic and real-world datasets demonstrate that DDF-HO consistently outperforms all baseline methods by a large margin, especially under Chamfer Distance, with about 80% leap forward. Codes are available at https://github.com/ZhangCYG/DDFHO.

==> sections/3method.tex <==
\section{Method}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/Pipeline.pdf}
    \caption{\textbf{Overview of DDF-HO.}
    }
    \label{fig:pipeline}
\end{figure*}

\subsection{Preliminary for Directed Distance Field}
Recently, several works~\cite{aumentado2022representing,houchens2022neuralodf,yoshitake2023transposer} for depth rendering, single-image 3D reconstruction and 3D generative modelling have successfully demonstrated that Directed Distance Fields (DDF) can be an effective and powerful implicit representation for 3D data.
Let $\mathcal{O} \subset \mathcal{B}$ be a 3D object shape, where $\mathcal{B} \subset \mathbb{R}^3$ is a bounding volume acting as the domain of the field.
Given a point $p \in \mathcal{B}$ and a view direction $d \in \mathbb{S}^2$, we define a ray $l_{p,d}(t) = p + td$.
The ray is called \textit{visible} if there exists intersection with $\mathcal{O}$ for some $t > 0$.
A Binary Visibility Field (BVF) for $\mathcal{O}$ is constructed as $\xi(p, d) = \mathbb{I}(l_{p,d} \quad is \quad visible)$.
Thus, we refer to a directed point $(p,d)$ as \textit{visible} if $\xi(p, d) = 1$.
We then define a Directed Distance Field (DDF) as a non-negative scalar field $D:\mathcal{B} \times \mathbb{S}^2 \rightarrow \mathbb{R}_+$.
It maps any directed point $(p,d)$ to the minimum distance to $\mathcal{O}$, i.e. the first intersection of $l_{p,d}$ with $\mathcal{O}$.
After the definition of the field $D$ and $\xi$, any point $q(p,d) \in \mathcal{O}$ can be recovered by $q(p,d) = D(p,d)d + p$ for $(p,d)$ satisfying $\xi(p, d) = 1$.
As is demonstrated by \cite{aumentado2022representing,houchens2022neuralodf}, such DDF $D$ and BNF $\xi$ can be fitted by deep neural networks, which is the foundation of our method DDF-HO.
Moreover, \cite{aumentado2022representing,houchens2022neuralodf} provide several convenient ways to convert DDF and BNF to other 3D representation including point cloud, mesh and vanilla SDF.


\subsection{In-Hand Objects Reconstruction}
Given a single RGB image $I$ and $n$ sampled rays $\{p_i, d_i\}$ in space, DDF-HO aims at constructing a conditional DDF $D$ and corresponding BVF $\xi$ for arbitrary in-hand objects $\mathcal{O}$, and thus reconstructs the in-hand objects by decoding the field into explicit representations.

Specifically, we first use an off-the-shelf system \cite{rong2020frankmocap} to estimate the hand articulation $\theta_H$ and the corresponding camera pose $\theta_C$ for the input image, where $\theta_H$ is a parametric MANO model with 45-dimensional articulation parameter \cite{romero2022embodied} and $\theta_C$ is a 6-dimensional global rotation and translation along with a weak perspective camera.
Then, $n$ rays $\{p_i, d_i\}$ are sampled in space by uniformly selecting the locations and directions.

Our hand-aware positional embedder $\phi(p, d, \theta_H)$ is utilized for extracting information of hand articulation joints around the intersected points with the estimated hand mesh for the sampled ray $(p, d), \xi(p, d) = 1$.
The key idea is that knowing the hand shape around the contact surface benefits the reconstruction of the in-hand object \cite{ye2022s}.
Corresponding hand-aware positional embedding $\mathcal{F}_\phi$ is extracted for the sampled $(p, d)$.
The object-aware visual embedder $\psi(p, d, \theta_C, I)$ with the proposed adaptive ray attention mechanism aggregates the features of the projected ray on the image plane, to ensure capturing the object feature thus to lead to more complete reconstruction.
Corresponding object-aware visual embedding $\mathcal{F}_\psi$ is extracted for the sampled $(p, d)$.

Finally, we use a MLP $\pi(p, d, \mathcal{F}_\phi, \mathcal{F}_\psi)$ to fit the conditional directed distance field, with the input $(p, d)$, as well as the concatenated hand-aware feature $\mathcal{F}_\phi$ and object-aware feature $\mathcal{F}_\psi$.
The output of $\pi(p, d, \mathcal{F}_\phi, \mathcal{F}_\psi)$ is the predicted value of DDF $D(p,d)$ and BVF $\xi(p,d)$.
Thus, the final in-hand object reconstruction result can be decoded by the predicted DDF and BVF and converted into other representation conveniently.


\subsection{Hand-Object-Conditioned Directed Distance Field}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/DDF_Attention.pdf}
    \caption{\textbf{Left: sampling space comparison of SDF against DDF. Right: Details of adaptive ray attention mechanism.}
    }
    \label{fig:DDF_Attention}
\end{figure*}

Powerful DDF representation enables more effective hand-aware and object-aware embeddings and leads to more accurate in-hand object reconstruction.

First, sampled points for SDF representation for an object must stick close to the object surface as much as possible, or the neural network may produce degenerated results and give noisy SDF predictions \cite{park2019deepsdf}.
However, such strict limitation for points sampling dose harm to the in-hand object reconstruction since the near-surface points are hard to capture the hand shape information to help the hand-held object reconstruction.
\cite{ye2022s} uses hand articulation feature around the sampled near-surface points to guide the SDF reconstruction, but the \textit{'feature around the sampled points'} is actually far from the hand surface.
Fig. \ref{fig:DDF_Attention} left shows that the SDF sampling space cannot cover the hand surface at all, leading degraded hand articulation feature sampling.
On the contrast, with DDF representation, we calculate the intersected points for a sampled $(p, d), \xi(p, d) = 1$ with the estimated hand surface represented by MANO model.
The intersected hand articulation feature is regared as the hand-aware positional embedding $\mathcal{F}_\phi$, which is one of the condition for the DDF prediction network.

Second, SDF representation only has sampled points without the guidance of ray directions.
Therefore, previous SDF method \cite{ye2022s} only projects the 3D sample points to corresponding image plane and gets the interpolated 2D feature as the visual feature for in-hand object reconstruction.
This approach is primitive and seems not effective in most cases when the project sampled point does not locate on the 2D object surface.
In fact, the sampled points of SDF representation are naturally out of the object surface, so that such feature extraction strategy cannot yield correct visual object feature.
Nevertheless, the exploitation of DDF representation enables aggregating visual features along the projected rays, which ensures capturing visual object feature since each ray with $(p, d), \xi(p, d) = 1$ must pass through the object.
We propose an adaptive ray attention mechanism for this object-aware visual embedding $\mathcal{F}_\psi$ which is discussed detailedly in Sec. \ref{attention}.

After get hand-aware $\mathcal{F}_\phi$ and object-aware $\mathcal{F}_\psi$, we use a MLP $\pi(p, d, \mathcal{F}_\phi, \mathcal{F}_\psi)$ to fit the hand-object-conditioned directed distance field, i.e. to predict the value of DDF $D(p,d)$ and BVF $\xi(p,d)$.
The 8-layer MLP network architecture refers to \cite{mildenhall2021nerf, houchens2022neuralodf}.
The input 5-dimensional directed point $(p, d)$ is positional encoded by $\gamma$ function as \cite{mildenhall2021nerf}.
BVF value is output after the 3rd layer to leave the network capacity for the harder depth estimation task.
We also include a skip connection of the input directed point to the 4th layer to guide the DDF prediction.
The loss functions of the conditional directed distance field network consist of depth objective $\mathcal{L}_D = \xi|\hat{D} - D|$ and visibility objective $\mathcal{L}_\xi = BCE(\hat{\xi}, \xi)$.
The final loss is written as $\mathcal{L} = \mathcal{L}_D + \lambda \mathcal{L}_\xi$, where $\lambda$ is a balanced factor.



\subsection{Adaptive Ray Attention} \label{attention}
Previous SDF-based methods \cite{ye2022s} attempts to aggregate features within a local patch centered around the projection of the sampled points in the SDF sampling space, which does not lie on the object surface.
Therefore, such feature aggregation technique actually extracts features of the background with large probability and lacks the information of the corresponding intersection point on the object surface, which plays significant role for in-hand object reconstruction.
With the help of DDF representation, our DDF-HO constructs the object-aware embedding $\mathcal{F}_\psi$ with a novel adaptive ray attention mechanism, considering visual feature aggregation along the projected ray and ensuring the information extraction for object surface.

Given an oriented point $(p, d)$, we use the estimated camera pose $\theta_C$ to project the line $l_{p, d}$ to the image plane and get $l_{p, d}^i$.
Then, $N_l$ points are sampled on $l_{p, d}^i$ from the projected start point $p_i$ with equal intervals $v$.
Thus, the start point feature $F_{p_i}^{vis}$ and a ray feature set $\mathcal{F}_{vis}^{ray} = \{F_{p_i + v}^{vis}, F_{p_i + 2v}^{vis}, \cdots F_{p_i + N_lv}^{vis}\}$ are constructed.
We utilize a cross-attention mechanism \cite{vaswani2017attention} for the adaptive ray feature fusion by
\begin{equation}
Q = W_q F_{p_i}^{vis}, \quad K=V=\mathcal{F}_{vis}^{ray},\quad
F_{vis}^{fused}  = Softmax(Q K^T)V.
\end{equation}
\begin{equation}
F_\psi = F_{p_i}^{vis} + F_{vis}^{fused}.
\end{equation}
Here, we use the incremental attention for $F_\psi$, which is demonstrated to be more effective by \cite{}.
Therefore, the object-aware visual embedding $F_\psi$ is generated by fusing the ray feature adaptively.
$F_\psi$ can provide the conditional DDF regressor $\pi(p, d, \mathcal{F}_\phi, \mathcal{F}_\psi)$ with more heuristic information containing the object surface, thus leading to more accurate reconstruction.


==> sections/4exp.tex <==
\section{Experiments}

\subsection{Experimental Setup} \label{setup}
\textbf{Datasets.}
A synthetic dataset ObMan \cite{hasson2019learning} and two real-world datasets HO3D(v2) \cite{hampali2020honnotate} with MOW \cite{cao2021reconstructing} are utilized to evaluate DDF-HO in various scenarios.
ObMan consists of 8 categories of 2772 objects from ShapeNet \cite{chang2015shapenet}, with 21K grasps generated by GraspIt \cite{miller2004graspit}.
The grasped objects are rendered over random backgrounds through Blender.
We follow \cite{hasson2019learning,ye2022s} to split the training and testing set.
HO3D(v2) \cite{hampali2020honnotate} contains 77,558 images from 68 sequences with 10 different persons manipulating 10 different YCB objects \cite{calli2015ycb}.
The pose annotations are yielded by multi-camera optimization pipelines.
We follow \cite{hampali2020honnotate} to split training and testing set.
MOW \cite{cao2021reconstructing} comprises a total of  442 images and 121 object templates, collected from in-the-wild hand-object interaction datasets \cite{damen2018scaling,shan2020understanding}.
The approximated ground truths are generated via a single-frame optimization method \cite{cao2021reconstructing}.
The training and testing split remain the same as the released code of \cite{ye2022s}.

\textbf{Evaluation Metrics.}
We first refer \cite{aumentado2022representing} to convert DDF representation to point cloud and get the sampled point cloud from the corresponding ground truth mesh.
Following \cite{ye2022s}, we report Chamfer Distance (CD), F-score at 5mm threshold (F-5) and 10mm threshold (F-10) of the converted object point cloud, which reflects the quality of hand-held object reconstruction.

\textbf{Baselines.}
Three baselines without needs of known object templates, i.e. to predict hand-held object shape directly from a single RGB input, are taken into consideration to make fair comparison with our DDF-HO.
The baselines include Atlas-Net \cite{groueix2018papier} based HO \cite{hasson2019learning}, implicit field based GF \cite{karunratanakul2020grasping} and SDF based IHOI \cite{ye2022s}. 

\textbf{Implementation Details.}
We use the same off-line systems \cite{hasson2019learning, rong2020frankmocap} as \cite{ye2022s} to estimate the hand and camera poses.
% ObMan dataset and \cite{rong2020frankmocap} for HO3D(v2) and MOW dataset.
% The same adopted off-line systems ensure the fairness of comparison with \cite{ye2022s} and other baselines.
We also adopt a ResNet34 \cite{he2016deep} to extract a 5-layer visual feature pyramid, which keeps the same with \cite{ye2022s}.
The number of sampled points $K_l$ is set to 8 and number of multi-head attention is 2 for Adaptive Ray Attention technique.
$K_{3D}$ for $\mathcal{F}^{\mathcal{L}}_{3D}\}$ introduced in Sec. \ref{HandObjectInteraction} is selected as 8.
DDF-HO is trained end-to-end with an Adam optimizer with learning rate 1e-4 on ObMan for 100 epochs.
Following \cite{ye2022s}, we use the network weight learned on ObMan to initialize the training on HO3D(v2) and MOW.
Training on HO3D(v2) and MOW are optimized by an Adam optimizer with learning rate 1e-5 for another 100 and 10 epochs respectively following \cite{ye2022s}.
The weighting factor of the loss for DDF-HO $\lambda_1, \lambda_2$ is set to 5.0 and 0.5 respectively.
During evaluation, we convert DDF representation to point cloud, while during visualization, we convert DDF to mesh.
The strategy for representation transformation is introduced in the Supplementary Material.

\subsection{Evaluation on Synthetic Scenarios}\label{obman}

\begin{wraptable}{r}{6.0cm}
\begin{center}
\begin{tabular}{c|ccc}
\hline
Method            & F-5 $\uparrow$      & F-10 $\uparrow$       & CD $\downarrow$ \\
\hline
HO \cite{hasson2019learning} &0.23  &0.56  &0.64  
\\
GF \cite{karunratanakul2020grasping} &0.30   &0.51   &1.39   
 \\
IHOI \cite{ye2022s} &0.42   &0.63   &1.02   \\
Ours        &\textbf{0.55}  &\textbf{0.67}  &\textbf{0.14}  \\
\hline
\end{tabular}
\end{center}
\caption{Metrics on ObMan \cite{hasson2019learning} dataset. 
Overall best results are \textbf{in bold}.
}
\label{tab:obman}
\end{wraptable}


\iffalse
\begin{table}[t]
\begin{center}
\begin{tabular}{c|cccccccccc}
\hline
Metrics     &Methods& Bottle      &Bowl        &Camera &Can &Cellphone &Jar &Knife &Remote Control &Mean \\
\hline
\multirow{2}{*}{F-5 $\uparrow$} &IHOI \cite{ye2022s} &0.52 &0.35 &0.34 &0.51 &0.43 &0.40 &0.28 &0.38 &0.42\\
&Ours &\textbf{0.61} &\textbf{0.56} &\textbf{0.50} &\textbf{0.65} &\textbf{0.58} &\textbf{0.53} &\textbf{0.46} &\textbf{0.52} &\textbf{0.55}\\
\hline
\multirow{2}{*}{F-10 $\uparrow$}
&IHOI \cite{ye2022s} &\textbf{0.73} &0.56 &0.57 &0.72 &0.63 &0.61 &0.46 &0.59 &0.63\\
&Ours &\textbf{0.73} &\textbf{0.70} &\textbf{0.64} &\textbf{0.79} &\textbf{0.68} &\textbf{0.66} &\textbf{0.56} &\textbf{0.63} &\textbf{0.67}\\
\hline
\multirow{2}{*}{CD $\downarrow$}
&IHOI \cite{ye2022s} &0.34 &1.54 &0.88 &0.32 &0.94 &0.81 &4.12 &1.11 &1.02\\
&Ours &\textbf{0.10} &\textbf{0.15} &\textbf{0.14} &\textbf{0.09} &\textbf{0.13} &\textbf{0.13} &\textbf{0.29} &\textbf{0.18} &\textbf{0.14}\\
\hline
\end{tabular}
\end{center}
\caption{Metrics on ObMan \cite{hasson2019learning} dataset. 
Overall best results are \textbf{in bold}.
}
\label{tab:obman_cat}
\end{table}
\fi

\input{sections/zhexian}

Evaluation on synthetic large-scale ObMan dataset demonstrates DDF-HO is enabled for more accurate hand-held object reconstruction results with the assistance of suitable DDF representation.
DDF-HO presents state-of-the-art performance in all three metrics of F-5, F-10 and CD.
Specifically, we have $13\%$ and $4\%$ leaps forward the current top-performing SDF-based IHOI on F-5 and F-10 respectively. 
The overwhelming performance on F-5 metric illustrates that DDF-HO can conduct more exquisite hand-held object reconstruction with the help of more suitable ray-based feature aggregation technique.
Notably, the CD metric of DDF-HO is decreased by $85\%$ compared with IHOI and $77\%$ with HO.
This demonstrates our predicted object surface contains much less outliers.

Fig. \ref{} shows visulization results of DDF-HO, with neater and more accurate hand-held object surface reconstruction.


\subsection{Evaluation on Real-world Scenarios}


Besides synthetic scenarios, we also conduct experiments to evaluate DDF-HO performance to handle real-world human object interactions on two real-world datasets HO3D(v2) and MOW.
Tab. \ref{tab:ho3d} exhibits the evaluation results on HO3D(v2) after finetuning (relative settings introduced in Sec. \ref{setup}) as well as zero-shot generalization results where we directly conduct inference on HO3D(v2) with the weights learned on ObMan.
Meanwhile, Tab. \ref{tab:mow} shows corresponding results on MOW.

Our method after real-world finetuning achieves the state-of-the-art on two datasets respectively.
On HO3D(v2), we have a considerable leap forward compared with IHOI and other methods, with increased F-5 by $6\%$, F-10 by $3\%$ and significantly decreased CD by $73\%$.
While on MOW, 

Moreover, the zero-shot experiments illustrates that DDF-HO is enabled stronger ability for synthetic-to-real generalization.
Specifically, on HO3D(v2), DDF-HO yields superior F-5 by $7\%$, F-10 by $5\%$ and decreased CD by $82\%$.
On MOW, 
The zero-shot experiments demonstrate that even trained only on synthetic dataset, DDF-HO still get decent results on real-world scenario, thanks to the generic representation ability of DDF for hand-object interaction modelling.

Fig. \ref{} shows the visualization comparison results on HO3D(v2).

\begin{table}[t]
\begin{center}
\begin{tabular}{c|ccc|ccc}
\hline
Method            & F-5 $\uparrow$      & F-10 $\uparrow$       & CD $\downarrow$  & F-5 $\uparrow$      & F-10 $\uparrow$       & CD $\downarrow$\\
\hline
HO \cite{hasson2019learning} &0.08  &0.19 &4.60  &0.05  &0.14  &6.03
\\
GF \cite{karunratanakul2020grasping} &0.09  &0.21  &5.23 &0.07  &0.16  &6.25  
 \\
IHOI \cite{ye2022s} &0.21   &0.38   &1.99  &0.17  &0.31  &4.17 \\
Ours        &\textbf{0.28}  &\textbf{0.42}  &\textbf{0.55}  &\textbf{0.24}  &\textbf{0.36}  &\textbf{0.73}\\
\hline
\end{tabular}
\end{center}
\caption{Metrics on HO3D(v2) \cite{hampali2020honnotate} dataset with finetuning (left) and zero-shot generalization from ObMan \cite{hasson2019learning} dataset (right). 
Overall best results are \textbf{in bold}.
}
\label{tab:ho3d}
\end{table}


\begin{table}[t]
\begin{center}
\begin{tabular}{c|ccc|ccc}
\hline
Method            & F-5 $\uparrow$      & F-10 $\uparrow$       & CD $\downarrow$  & F-5 $\uparrow$      & F-10 $\uparrow$       & CD $\downarrow$\\
\hline
IHOI \cite{ye2022s} &0.10  &0.19  &7.83 &0.09   &0.17   &8.43   \\
Ours        &\textbf{0.16}  &\textbf{0.22}  &\textbf{1.59} &\textbf{0.14}  &\textbf{0.19}  &\textbf{1.89} \\
\hline
\end{tabular}
\end{center}
\caption{Metrics on MOW \cite{cao2021reconstructing} dataset, with the setting of finetuning (left) and zero-shot generalization from ObMan \cite{hasson2019learning} dataset (right).
Overall best results are \textbf{in bold}.
}
\label{tab:mow}
\end{table}


\subsection{Ablation Studies}

\begin{table}[t]
\begin{center}
\begin{tabular}{ccc|ccc|ccc}
\hline
RFA &IHF &SYM & F-5 $\uparrow$      & F-10 $\uparrow$       & CD $\downarrow$ & F-5 $\uparrow$      & F-10 $\uparrow$       & CD $\downarrow$\\
\hline
$\times$ &$\times$ & $\times$ &0.45  &0.60  &0.22 &0.24 &0.38 &0.62
\\
$\checkmark$ &$\times$ & $\times$ &0.50   &0.64   &0.17 &0.26 &0.39 &0.58
 \\
$\checkmark$ &$\checkmark$ & $\times$ &0.55   &0.67   &0.14  &0.28 &0.42 &0.55 \\
$\checkmark$ &$\checkmark$ & $\checkmark$   &\textbf{0.57}  &\textbf{0.68}  &\textbf{0.13}  & & &\\
\hline
\end{tabular}
\end{center}
\caption{Ablation studies for key assets of DDF-HO on ObMan \cite{hasson2019learning} (left) and HO3D(v2) \cite{hampali2020honnotate} dataset (right). 
}
\label{tab:ablation}
\end{table}

\begin{table}[t]
\begin{center}
\begin{tabular}{c|ccc|ccc}
\hline
Noise & F-5 $\uparrow$      & F-10 $\uparrow$       & CD $\downarrow$ & F-5 $\uparrow$      & F-10 $\uparrow$       & CD $\downarrow$\\
\hline
Pred & 0.55  &0.67  &0.14 & & &
\\
Pred+$\sigma=0.1$&   &  & & & &
 \\
Pred+$\sigma=0.5$ &   &   &  & & & \\
GT &  &  & & & &
\\
GT+$\sigma=0.1$&   &  & & & &
 \\
GT+$\sigma=0.5$ &   &   &  & & & \\
\hline
\end{tabular}
\end{center}
\caption{Ablation studies for input hand pose on ObMan \cite{hasson2019learning} (left) and HO3D(v2) \cite{hampali2020honnotate} dataset (right). 
}
\label{tab:noise}
\end{table}

Three key assets of DDF representation are ablated on ObMan and HO3D(v2) dataset, including Ray-Based Feature Aggregation (RFA), Intersection-aware Hand Feature (IHF) and Symmetry Loss (SYM), with results shown in Tab. \ref{tab:ablation}.
On ObMan, if we only substitute SDF representation to DDF without any change for feature aggregation (the 1st row), the result is slightly enhanced compared to the SDF-based IHOI (reported in Tab. \ref{tab:obman}) with $3\%$ promotion in F-5 metric.
This illustrates that although DDF is more suitable for represent hand-object interaction (with almost $80\%$ decrease of CD metric), more sophisticated designs towards proper feature aggregation are necessitated.
Thus, after utilizing RFA technique (Sec. \ref{rayfeaturesection}) considering the representation characteristics of sampled rays, F-5 metric increases by another $5\%$ and F-10 enhances by $4\%$.
Moreover, adding IHF (Sec. \ref{HandObjectInteraction}) which emphasizes to model hand-object interaction locally makes F-5 promote by $3\%$ and F-10 by $2\%$.
It indicates that considering the intersection information of hand can assist the accuracy of hand-held object reconstruction.
Finally, the SYM loss helps DDF-HO perceive the symmetry nature of the majority of everyday objects and handle the self-occluded scenarios caused by hands, with another enhancement of F-5 by $2\%$ and F-10 by $1\%$.
Meanwhile, on real-world HO3D(v2) dataset, RFA, IHF and SYM modules plays similar roles as on ObMan.

We also ablate the influence of input hand pose on DDF-HO, by adding Gaussian noise on the input estimated hand poses (Pred, as the experiment settings in Sec. \ref{obman}) or ground truth hand poses (GT).
The ablation results (Tab. \ref{tab:noise}) on ObMan and HO3D(v2) demonstrate the robustness of DDF-HO for handling noisy input hand poses.




==> sections/zhexian.tex <==
\definecolor{darkyellow}{RGB}{232, 155, 0}

\begin{figure}


\begin{tikzpicture}

\begin{groupplot}[
    group style={
      {group size=3 by 1}},
    height=0.35\textwidth,width=0.38\textwidth,y label style={below=1mm}, x label style={below=-2.5mm}, title style={below=-2mm}
    ]

    \nextgroupplot[title=Category ID $\sim$ F-5$\uparrow$,  
    % legend style={font=\fontsize{4}{5}\selectfont, line width=0.1},
    legend style={at={(2.90,0.6)},
      anchor=south,legend columns=1, },
    % legend pos=north west,
    ] 

\addplot[
    color=darkyellow,
    mark=x,
    ]
    coordinates {
    (0, 0.52)
    (1, 0.35)
    (2, 0.34)
    (3, 0.51)
    (4, 0.43)
    (5, 0.40)
    (6, 0.28)
    (7, 0.38)
    };
    \addlegendentry{IHOI~\cite{ye2022s}}
    
    \addplot[
    color=blue,
    mark=o,
    ]
    coordinates {
    (0, 0.61)
    (1, 0.56)
    (2, 0.50)
    (3, 0.65)
    (4, 0.58)
    (5, 0.53)
    (6, 0.46)
    (7, 0.52)
    };
    \addlegendentry{DDF-HO}

% \end{axis}
    \nextgroupplot[title=Category ID $\sim$ F-10$\uparrow$]
\addplot[
    color=darkyellow,
    mark=x,
    ]
    coordinates {
    (0, 0.73)
    (1, 0.56)
    (2, 0.57)
    (3, 0.72)
    (4, 0.63)
    (5, 0.61)
    (6, 0.46)
    (7, 0.59)
    };
   % \addlegendentry{}
    
    \addplot[
    color=blue,
    mark=o,
    ]
    coordinates {
    (0, 0.73)
    (1, 0.70)
    (2, 0.64)
    (3, 0.79)
    (4, 0.68)
    (5, 0.66)
    (6, 0.56)
    (7, 0.63)
    };
    % \addlegendentry{Uy \textit{et al.}~\cite{uy2021joint}}

    
    \nextgroupplot[title=Category ID $\sim$ CD$\downarrow$]
    \addplot[
    color=darkyellow,
    mark=x,
    ]
    coordinates {
    (0, 0.34)
    (1, 1.54)
    (2, 0.88)
    (3, 0.32)
    (4, 0.94)
    (5, 0.81)
    (6, 4.12)
    (7, 1.11)
    };
    % \addlegendentry{ShapeFlow~\cite{jiang2020shapeflow}}
    
    \addplot[
    color=blue,
    mark=o,
    ]
    coordinates {
    (0, 0.10)
    (1, 0.15)
    (2, 0.14)
    (3, 0.09)
    (4, 0.13)
    (5, 0.13)
    (6, 0.29)
    (7, 0.18)
    };
    % \addlegendentry{Uy \textit{et al.}~\cite{uy2021joint}}


    % \addlegendentry{Ours}
  \end{groupplot}

\end{tikzpicture}
\vspace{-0.3cm}
\caption{Reconstruction quality comparisons on Obman~\cite{hasson2019learning} by category. From 0 to 7, we demonstrate the results of IHOI~\cite{ye2022s} \textit{vs} DDF-HO on the categories: {Bottle, Bowl, Camera, Can, Cellphone, Jar, Knife, Remote Control} sequentially.
DDF-HO consistently outperforms IHOI.}
\label{fig:partial_result}
\end{figure}


